Transferability-Guided Cross-Domain Cross-Task Transfer Learning

We propose two novel transferability metrics F-OTCE (Fast Optimal Transport based Conditional Entropy) and JC-OTCE (Joint Correspondence OTCE) to evaluate how much the source model (task) can benefit the learning of the target task and to learn more transferable representations for cross-domain cross-task transfer learning. Unlike the existing metric that requires evaluating the empirical transferability on auxiliary tasks, our metrics are auxiliary-free such that they can be computed much more efficiently. Specifically, F-OTCE estimates transferability by first solving an Optimal Transport (OT) problem between source and target distributions, and then uses the optimal coupling to compute the Negative Conditional Entropy between source and target labels. It can also serve as a loss function to maximize the transferability of the source model before finetuning on the target task. Meanwhile, JC-OTCE improves the transferability robustness of F-OTCE by including label distances in the OT problem, though it may incur additional computation cost. Extensive experiments demonstrate that F-OTCE and JC-OTCE outperform state-of-the-art auxiliary-free metrics by 18.85% and 28.88%, respectively in correlation coefficient with the ground-truth transfer accuracy. By eliminating the training cost of auxiliary tasks, the two metrics reduces the total computation time of the previous method from 43 minutes to 9.32s and 10.78s, respectively, for a pair of tasks. When used as a loss function, F-OTCE shows consistent improvements on the transfer accuracy of the source model in few-shot classification experiments, with up to 4.41% accuracy gain.

==> images/fig_otce_finetune.tex <==
\begin{figure}[t]
\centering
%\def\svgwidth{0.9\linewidth}
%\includesvg{images/otce_finetune_black}

\includegraphics[width=0.8\linewidth]{images/pipeline_of_OTCE_FT.png}
\caption{The pipeline of our OTCE-based finetune method.}
\label{fig: otce finetune}
%\vspace{-0.4cm}
\end{figure}


==> section/biography.tex <==

%\newpage

%\vspace{-8cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/tanyang.jpg}}] {Yang Tan}
(Student Member, IEEE) received his BE degree from the School of Electronic Engineering, Xidian University, Xi’an, China, in 2017, and his MS degree from the School of Data and Computer Science, Sun Yat-sen University, Guangzhou, China, in 2019. He is currently working toward the PhD degree at the Tsinghua-Berkeley Shenzhen Institute (TBSI), Tsinghua University. His research interests include transfer learning and its application in computer vision. 

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/enmingzhang.jpg}}] {Enming Zhang} is currently working toward the PhD degree at the Tsinghua Shenzhen International Graduate School, Tsinghua University. His main research interests include transfer learning and domain adaptation.
	
\end{IEEEbiography}

%\vspace{-8cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/yangli.png}}]{Yang Li}
 (Member, IEEE) received her B.A. degree in computer science and mathematics from Smith College in 2011, and her Ph.D. degree in computer science from Stanford University in 2017. She had been a postdoctoral fellow at Tsinghua-Berkeley Shenzhen Institute, China from 2017-2019. Since 2019, she has been an assistant professor at the Data Science and Information Technology Research Center of Tsinghua-Berkeley Shenzhen Institute.  Her research interests include transfer learning, representation learning with multiple tasks and domains, spatial data analysis and geometric algorithms.  

\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
\newpage

%\vspace{-15cm}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/shaolunhuang.png}}]{Shao-Lun Huang}
(Member, IEEE) received the B.S. degree with honor in 2008 from the Department of Electronic Engineering, National Taiwan University, Taiwan, and the M.S. and Ph.D. degree in 2010 and 2013 from the Department of Electronic Engineering and Computer Sciences, Massachusetts Institute of Technology. From 2013 to 2016, he was working as a postdoctoral researcher jointly in the Department of Electrical Engineering at the National Taiwan University and the Department of Electrical Engineering and Computer Science at the Massachusetts Institute of Technology. Since 2016, he has joined Tsinghua-Berkeley Shenzhen Institute, where he is currently an associate professor. His research interests include information theory, communication theory, machine learning, and social networks.
\end{IEEEbiography}

%\vspace{10.2cm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{biography/xiaopingzhang.png}}]{Xiao-Ping Zhang} (Fellow, IEEE) received the BS and PhD degrees in electronic engineering from Tsinghua University, Beijing, China, in 1992 and 1996, respectively, and the MBA degree in finance, economics and entrepreneurship (with Hons.) from the University of Chicago Booth School of Business, Chicago, IL, USA. Since Fall 2000, he has been with the Department of Electrical, Computer and Biomedical Engineering, Ryerson University, Toronto, ON, Canada, where he is currently a professor and the Director of the Communication and Signal Processing Applications Laboratory. In 2015 and 2017, he was a visiting scientist with the Research Laboratory of Electronics, Massachusetts Institute of Technology, Cambridge, MA, USA. His research interests include sensor networks and IoT, machine learning, statistical signal processing, image and multimedia content analysis, and applications in Big Data, finance, and marketing. He is a Fellow of the Canadian Academy of Engineering, Fellow of the Engineering Institute of Canada. He was the recipient of the 2020 Sarwan Sahota Ryerson Distinguished Scholar Award, the Ryerson University highest honor for scholarly, research and creative achievements. He is selected as IEEE Distinguished Lecturer by the IEEE Signal Processing Society for the term 2020 to 2021, and by the IEEE Circuits and Systems Society for the term 2021 to 2022.

\end{IEEEbiography}



==> section/figure/fig_illustration_of_OTCE.tex <==
\begin{figure}[t]
	\centering
	\def\svgwidth{1.0\linewidth}
	\includesvg{images/OTCE}
	\caption{Illustration of previous auxiliary-based OTCE metric~\cite{OTCE}, where $\hat{W}_D$ and $\hat{W}_T$ denote the \textit{domain difference} and the \textit{task difference} respectively, and $\lambda_1, \lambda_2, b$ are learned coefficients from auxiliary tasks with known empirical transferability. }
	\label{fig: illustration of OTCE}
	%\vspace{-0.4cm}
\end{figure}


==> section/figure/fig_property_comparison.tex <==
\begin{figure}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{images/property_comparison_cut.pdf}
	\caption{Efficiency and accuracy comparisons among transferability metrics. We can conclude that $ \text{OTCE} < \text{JC-OTCE} < \text{F-OTCE}$ on efficiency and $ \text{OTCE} \approx \text{JC-OTCE} > \text{F-OTCE}$ on accuracy.}
	\label{fig:property comparison}
	%\vspace{-0.5cm}
\end{figure}

==> section/table/tab_metric_comparisons.tex <==
\begin{table}[t]
	\centering
\begin{minipage}{1.0\linewidth}

\centering
%\setlength\tabcolsep{4pt} 

\footnotesize

\caption{Properties of our proposed transferability metrics.}
\label{tab: metric property comparison}

\begin{tabular}{cccc}
\toprule
Property & OTCE~\cite{OTCE} & $\text{OTCE}_s$ & JC-OTCE \\
\midrule

Auxiliary-free & \XSolidBrush & \Checkmark & \Checkmark \\
\midrule
Efficiency & \multicolumn{3}{c}{$\text{OTCE}_s > \text{JC-OTCE} > \text{OTCE} $} \\
Accuracy & \multicolumn{3}{c}{$ \text{OTCE} \approx \text{JC-OTCE} > \text{OTCE}_s$} \\


\bottomrule

\end{tabular}

\end{minipage}
\end{table}



%\multirow{2} {*}{Image classification} & Empirical transferability & 858s (14.3min) \\

